SIR: Structured Image Representations for Explainable Robot Learning

Existing robot policies based on learned visual embeddings lack explicit structure and are sensitive to visual distractions. Thus, the representations that drive their behaviour are often opaque, making their decision-making process difficult to interpret. To address this, we introduce Structured Image Representations (SIR), a method that leverages Scene Graphs (SGs) as an intermediate representation for robot policy learning. Our approach first constructs a fully connected graph, using image-derived features as initial node representations. Then, a module learns to sparsify this graph end-to-end, creating a task-relevant sub-graph that is passed to the action generation model. This process makes our model intrinsically explainable. Evaluations on RoboCasa show that our sparse graph policies outperform image-based baselines on average with 19.5% vs 14.81% success rate. Most importantly, we show that the learned sparse graphs are a powerful tool for model analysis. By analysing when the model's sub-graph deviates from human expectation, such as by including distractor nodes or omitting key objects, we successfully uncover dataset biases, including spurious correlations and positional biases. https://github.com/intuitive-robots/SIR_Model

==> sec/stuff.tex <==
\begin{table*}[t]
\caption{The results represent success rate over 100 rollouts with 2 models trained on different seeds.}
\label{tab:homogeneous_tasks}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l|l|l|l}
\hline
& \shortstack{Feature \\ Input} & 
\shortstack{Pick and \\ Place} & 
\shortstack{Open/Close \\ Doors} & 
\shortstack{Open/Close \\ Drawers} & 
\shortstack{Twisting \\ Knobs} & 
\shortstack{Turning \\ Levers} & 
\shortstack{Pressing \\ Buttons} & 
\shortstack{Insertion} & 
Average \\
\hline
\multirow{9}{*}{\rotatebox{90}{\acs{mdt}}} & 
    B: Image & 1.19 & 25.13 & 49.75 & 7.25 & 23.67 & 17.0 & 4.75 & 14.81 \\
    & B: Point Clouds & 0.0 & 0.0 & 1.0 & 1.25 & 19.83 & 10.83 & 1.25 & 4.13  \\
    & B: I + P C & 0.56 & 25.25 & 44.75 & 5.5 & 20.67 & 15.17 & 2.25 & 13.25 \\
    \cline{2-10}
    & O: Image & 0.25 & 20.88 & 37.25 & 15.0 & 48.33 & 17.17 & 6.5 & 16.65 \\
    & O: BB + Label & 0.13 & 19.13 & 31.5 & 13.5 & 21.17 & 7.67 & 4.75 & 10.98 \\
    & O: BB + Image & 0.25 & 23.13 & 35.25 & 14.25 & 40.33 & 17.67 & 7.0 & 15.9 \\
    & O: Point Clouds & 0.06 & 11.38 & 29.25 & 18.5 & 30.33 & 9.67 & 2.25 & 11.08 \\
    & O: L + P C & 0.4 & 15.88 & 32.25 & 15.0 & 36.83 & 8.33 & 1.75 & 12.5 \\
    & O: I + P C & 0.25 & 19.38 & 40.75 & 8.5 & 40.83 & 16.0 & 6.25 & 15.04  \\
    \hline
    & O: Baseline: fully-connected{,} no sparsification{,} no node removal & 0.06 & 14.12 & 31.50 & 13.00 & 27.17 & 11.00 & 2.50 & 11.06 \\
    & O: Wie 1{,} aber ImgAsLAbel anstatt One-Hot-Encoding für Labels & 0.12 & 29.75 & 38.75 & 17.25 & 40.50 & 17.83 & 6.00 & 17.46 \\
    & O: Neu-Evaluierung von 2: using same y-bounds always & 0.06 & 28.62 & 39.25 & 14.00 & 40.00 & 18.83 & 4.75 & 16.98 \\
    & O: Nur Bilder{,} keine Graphen & 0.38 & 26.25 & 43.50 & 7.00 & 27.33 & 16.50 & 2.50 & 14.40 \\
    & O: Wie 4{,} aber SGATv2 (l0\_weight=0) & 0.06 & 21.38 & 37.25 & 14.00 & 43.00 & 16.50 & 1.75 & 15.44 \\
    & O: Wie 7{,} aber NodeConditioning (node\_cond\_dim=512) & 0.19 & 23.25 & 44.25 & 15.50 & 41.33 & 17.17 & 3.75 & 16.54 \\
    & O: Wie 8{,} aber use\_mlp\_first=True (input\_linear\_dim=512) anstatt NodeConditioning & 0.12 & 21.00 & 38.00 & 14.50 & 41.17 & 15.17 & 2.50 & 15.17 \\
    & O: Node-Scores (Transformer) - no additional losses & 0.00 & 8.50 & 23.50 & 6.75 & 29.17 & 13.83 & 3.50 & 9.60 \\
    & O: Node-Scores (Transformer{,} uniform\_dist\_weight=1e-4) & 0.00 & 7.75 & 18.25 & 8.50 & 31.67 & 11.83 & 2.75 & 9.19 \\
    & O: Node-Scores (Transformer{,} variance\_weight=1e-4) & 0.06 & 13.75 & 29.00 & 7.50 & 33.67 & 12.17 & 4.00 & 11.42 \\
    & O: Node-Scores (Transformer{,} sum\_mask\_weight=1e-6{,} target\_sum\_node\_probs=5) & 0.12 & 15.50 & 33.75 & 8.75 & 30.33 & 12.67 & 3.00 & 11.79 \\
    & O: Wie 7{,} aber l0\_weight=1e-5 & 0.12 & 24.50 & 43.25 & 15.25 & 43.50 & 15.83 & 3.00 & 16.67 \\
    & O: wie 7{,} aber l0\_weight=3e-7 & 0.06 & 24.75 & 42.75 & 16.50 & 43.67 & 14.00 & 2.75 & 16.52 \\
    & O: wie 9{,} aber input\_linear\_dim=57 & 0.12 & 21.75 & 39.50 & 9.25 & 35.00 & 14.67 & 5.50 & 14.40 \\
    & O: wie 11{,} aber uniform\_dist\_weight=1e-2 & 0.00 & 23.12 & 41.25 & 15.00 & 36.33 & 17.50 & 5.00 & 15.69 \\
    & O: wie 11{,} aber uniform\_dist\_weight=1e-1 & 0.19 & 25.12 & 39.75 & 11.25 & 43.00 & 17.83 & 4.75 & 16.50 \\
    & \shortstack{O: NodeCond(use\_node\_cond=only\_in\_coarsening\_and\_sparsification{,} \\ node\_cond\_dim=512)+Coarsening(uniform\_dist\_weight=1e-1)+SGAT(l0\_weight=0)} & 0.25 & 23.50 & 43.75 & 14.25 & 38.17 & 15.67 & 5.75 & 16.04 \\
    & \shortstack{O: NodeCond(use\_node\_cond=only\_in\_coarsening\_and\_sparsification{,} \\ node\_cond\_dim=512)+Coarsening(uniform\_dist\_weight=1e-2)+SGAT(l0\_weight=0)} & 0.12 & 22.38 & 43.25 & 10.75 & 36.33 & 17.67 & 3.75 & 15.33 \\
    & O: L/R PC (von CVPR-Paper) & 0.06 & 11.38 & 29.25 & 18.50 & 30.33 & 9.67 & 2.25 & 14.49 \\
    & O: L/R I+BB (von CVPR-Paper) & 0.25 & 23.13 & 35.25 & 14.25 & 40.33 & 17.67 & 7.00 & 19.70 \\
    & O: L/R L+BB (von CVPR-Paper) & 13.00 & 19.13 & 31.50 & 13.50 & 21.17 & 7.67 & 4.75 & 15.82 \\
    & O: Unnamed Model & 0.38 & 21.12 & 40.00 & 17.75 & 41.50 & 18.67 & 3.75 & 16.29 \\
    & O: Unnamed Model & 0.56 & 18.25 & 46.25 & 3.25 & 17.17 & 14.50 & 2.50 & 11.52 \\
    & O: Unnamed Model & 0.31 & 17.25 & 37.25 & 15.25 & 38.00 & 22.00 & 3.00 & 15.10 \\
    & O: Unnamed Model & 0.56 & 20.38 & 39.00 & 14.00 & 39.67 & 19.33 & 3.25 & 15.65 \\
    & O: Unnamed Model & 0.44 & 6.88 & 25.50 & 16.50 & 31.00 & 17.83 & 2.00 & 11.06 \\
    & O: Unnamed Model & 0.38 & 11.00 & 30.75 & 14.50 & 35.17 & 16.33 & 1.00 & 12.25 \\
    & O: Wie 22{,} aber variance\_weight=1e-4{,} target\_sum\_weight=5e-6{,} target\_sum\_node\_probs=6 & 0.06 & 25.87 & 36.75 & 19.25 & 36.67 & 17.83 & 5.00 & 16.23 \\
    & O: Wie 22{,} aber variance\_weight=1e-3{,} target\_sum\_weight=5e-5{,} target\_sum\_node\_probs=6 & 0.12 & 26.00 & 37.50 & 18.50 & 40.67 & 14.50 & 3.50 & 16.23 \\
    & O: -> schlechte Performance von 33(23)/34(24) liegt nicht an SGAT & 0.31 & 15.38 & 46.75 & 16.00 & 42.33 & 16.00 & 4.50 & 15.56 \\
\hline
\hline
\multirow{4}{*}{\rotatebox{90}{\acs{bc}}} & 
    B: Image &  &  &  &  &  &  &  &   \\
    \cline{2-10}
    & O: Image &  &  &  &  &  &  &  &  \\
    & O: BB + Label &  &  &  &  &  &  &  &  \\
    & O: BB + Image &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
}
\end{table*}

\begin{table*}[t]
\caption{Five most relevant nodes per task and model.} 
\label{tab:FiveMostRelevantNodesPerTaskAndModel}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l}
\shortstack{Task} & 
\multicolumn{2}{|c|}{TopK NR + soft histogram loss} & 
\multicolumn{2}{|c|}{Instruction grounded + NR + soft histogram loss} &
\multicolumn{2}{|c|}{threshold NR + soft histogram loss}\\
\hline
Seed & (1) & (2) & (1) & (2) & (1) & (2) \\
\hline
PnP  &  &  &  &  &  &  \\
\hline
PnPCabToCounter  & \shortstack{PandaMobile (1.000) \\ HingeCabinet (1.000) \\ Wall (0.947) \\ Counter (0.918) \\ SingleCabinet (0.844) } & \shortstack{PandaMobile (0.997) \\ Hood (0.985) \\ PandaGripper (0.893) \\ Toaster (0.763) \\ distr\_counter (0.689) } & \shortstack{SingleCabinet (1.000) \\ PandaMobile (1.000) \\ HingeCabinet (1.000) \\ Counter (1.000) \\ PandaGripper (0.985) } & \shortstack{HingeCabinet (1.000) \\ PandaMobile (1.000) \\ Counter (0.986) \\ PandaGripper (0.977) \\ SingleCabinet (0.936) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.964) \\ SingleCabinet (0.909) \\ Toaster (0.891) \\ FramedWindow (0.503) } & \shortstack{PandaMobile (1.000) \\ FramedWindow (0.950) \\ PandaGripper (0.912) \\ Sink (0.690) \\ Toaster (0.672) } \\
\hline
PnPCounterToCab  & \shortstack{PandaMobile (1.000) \\ HingeCabinet (1.000) \\ Wall (0.992) \\ SingleCabinet (0.907) \\ Counter (0.836) } & \shortstack{PandaMobile (0.994) \\ Toaster (0.952) \\ obj (0.829) \\ PandaGripper (0.822) \\ distr\_counter (0.747) } & \shortstack{HingeCabinet (1.000) \\ PandaMobile (1.000) \\ Counter (1.000) \\ PandaGripper (0.995) \\ SingleCabinet (0.963) } & \shortstack{Counter (1.000) \\ PandaMobile (0.999) \\ PandaGripper (0.996) \\ HingeCabinet (0.917) \\ SingleCabinet (0.914) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.925) \\ SingleCabinet (0.924) \\ Toaster (0.882) \\ FramedWindow (0.870) } & \shortstack{PandaMobile (0.997) \\ PandaGripper (0.929) \\ Toaster (0.672) \\ FramedWindow (0.575) \\ SingleCabinet (0.569) } \\
\hline
PnPCounterToMicrowave  & \shortstack{Microwave (0.999) \\ PandaMobile (0.999) \\ Oven (0.849) \\ container (0.791) \\ Fridge (0.714) } & \shortstack{PandaMobile (0.988) \\ obj\_container (0.892) \\ obj (0.795) \\ distr\_counter (0.768) \\ PandaGripper (0.734) } & \shortstack{PandaMobile (0.999) \\ Microwave (0.999) \\ PandaGripper (0.951) \\ Counter (0.951) \\ obj (0.657) } & \shortstack{PandaMobile (1.000) \\ Microwave (0.998) \\ Counter (0.982) \\ PandaGripper (0.980) \\ obj (0.662) } & \shortstack{Stovetop (1.000) \\ PandaMobile (0.983) \\ PandaGripper (0.829) \\ obj\_container (0.800) \\ container (0.649) } & \shortstack{PandaMobile (0.998) \\ PandaGripper (0.749) \\ obj\_container (0.679) \\ FramedWindow (0.568) \\ Oven (0.526) } \\
\hline
PnPCounterToSink  & \shortstack{PandaMobile (1.000) \\ Sink (0.974) \\ CoffeeMachine (0.937) \\ Wall (0.915) \\ Counter (0.874) } & \shortstack{PandaMobile (0.997) \\ obj (0.815) \\ distr\_counter (0.803) \\ PandaGripper (0.709) \\ distr\_sink (0.704) } & \shortstack{PandaMobile (0.998) \\ Counter (0.997) \\ Sink (0.997) \\ PandaGripper (0.933) \\ obj (0.824) } & \shortstack{PandaMobile (1.000) \\ Counter (0.998) \\ Sink (0.992) \\ PandaGripper (0.973) \\ obj (0.861) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.832) \\ FramedWindow (0.726) \\ distr\_counter (0.601) \\ WallAccessory (0.509) } & \shortstack{PandaMobile (1.000) \\ CoffeeMachine (0.912) \\ PandaGripper (0.823) \\ WallAccessory (0.564) \\ FramedWindow (0.461) } \\
\hline
PnPCounterToStove  & \shortstack{Microwave (1.000) \\ PandaMobile (0.997) \\ Wall (0.954) \\ Drawer (0.943) \\ Stovetop (0.939) } & \shortstack{PandaMobile (0.982) \\ obj\_container (0.961) \\ obj (0.836) \\ PandaGripper (0.819) \\ WallAccessory (0.444) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.989) \\ Counter (0.984) \\ Stove (0.981) \\ obj (0.900) } & \shortstack{PandaMobile (1.000) \\ Counter (0.999) \\ PandaGripper (0.999) \\ Stove (0.997) \\ obj (0.937) } & \shortstack{PandaMobile (0.987) \\ Fridge (0.957) \\ PandaGripper (0.882) \\ obj\_container (0.823) \\ WallAccessory (0.601) } & \shortstack{PandaMobile (0.995) \\ obj\_container (0.892) \\ PandaGripper (0.883) \\ CoffeeMachine (0.752) \\ WallAccessory (0.710) } \\
\hline
PnPMicrowaveToCounter  & \shortstack{PandaMobile (1.000) \\ Microwave (1.000) \\ Oven (0.865) \\ Fridge (0.805) \\ Wall (0.799) } & \shortstack{PandaMobile (0.976) \\ container (0.839) \\ obj (0.776) \\ PandaGripper (0.769) \\ distr\_counter (0.606) } & \shortstack{PandaMobile (0.993) \\ Microwave (0.976) \\ PandaGripper (0.945) \\ Counter (0.940) \\ obj (0.799) } & \shortstack{Microwave (0.998) \\ Counter (0.964) \\ PandaMobile (0.961) \\ PandaGripper (0.951) \\ obj (0.845) } & \shortstack{Sink (1.000) \\ PandaMobile (0.997) \\ PandaGripper (0.887) \\ container (0.750) \\ Oven (0.720) } & \shortstack{PandaMobile (0.988) \\ PandaGripper (0.733) \\ Oven (0.713) \\ container (0.553) \\ obj (0.394) } \\
\hline
PnPSinkToCounter  & \shortstack{PandaMobile (1.000) \\ Sink (0.997) \\ Wall (0.955) \\ FramedWindow (0.842) \\ Counter (0.792) } & \shortstack{PandaMobile (0.987) \\ container (0.916) \\ PandaGripper (0.877) \\ distr\_counter (0.736) \\ obj (0.717) } & \shortstack{obj (1.000) \\ Sink (0.999) \\ PandaMobile (0.999) \\ Counter (0.991) \\ PandaGripper (0.971) } & \shortstack{PandaMobile (1.000) \\ Counter (0.981) \\ Sink (0.970) \\ obj (0.947) \\ PandaGripper (0.933) } & \shortstack{PandaMobile (0.999) \\ FramedWindow (0.949) \\ PandaGripper (0.818) \\ WallAccessory (0.685) \\ container (0.640) } & \shortstack{Microwave (1.000) \\ PandaMobile (1.000) \\ PandaGripper (0.805) \\ container (0.681) \\ FramedWindow (0.666) } \\
\hline
PnPStoveToCounter  & \shortstack{Microwave (1.000) \\ PandaMobile (1.000) \\ Stovetop (0.888) \\ Wall (0.881) \\ Counter (0.638) } & \shortstack{PandaMobile (0.991) \\ container (0.984) \\ PandaGripper (0.880) \\ Dishwasher (0.621) \\ HingeCabinet (0.507) } & \shortstack{PandaMobile (1.000) \\ Stove (1.000) \\ Counter (1.000) \\ PandaGripper (0.999) \\ obj (0.939) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.999) \\ Stove (0.998) \\ Counter (0.990) \\ obj (0.977) } & \shortstack{PandaMobile (0.995) \\ PandaGripper (0.845) \\ container (0.843) \\ Stove (0.761) \\ CoffeeMachine (0.667) } & \shortstack{PandaMobile (0.993) \\ container (0.849) \\ PandaGripper (0.805) \\ WallAccessory (0.543) \\ Stove (0.474) } \\
\hline
Door  &  &  &  &  &  &  \\
\hline
OpenSingleDoor  & \shortstack{PandaMobile (0.979) \\ Wall (0.855) \\ Microwave (0.802) \\ PandaGripper (0.759) \\ Counter (0.672) } & \shortstack{Microwave (0.989) \\ FramedWindow (0.972) \\ PandaMobile (0.841) \\ Oven (0.835) \\ PandaGripper (0.831) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.976) \\ CoffeeMachine (0.302) \\ Toaster (0.249) \\ OmronMobileBase (0.215) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.994) \\ HingeCabinet (0.324) \\ Microwave (0.303) \\ Box (0.267) } & \shortstack{PandaMobile (0.999) \\ FramedWindow (0.998) \\ PandaGripper (0.870) \\ distr\_counter\_3 (0.732) \\ Oven (0.631) } & \shortstack{PandaMobile (0.979) \\ FramedWindow (0.949) \\ PandaGripper (0.818) \\ Microwave (0.750) \\ distr\_counter\_2 (0.638) } \\
\hline
OpenDoubleDoor  & \shortstack{PandaMobile (0.996) \\ Wall (0.990) \\ HingeCabinet (0.944) \\ PandaGripper (0.861) \\ Counter (0.793) } & \shortstack{PandaGripper (0.904) \\ HingeCabinet (0.901) \\ PandaMobile (0.891) \\ Sink (0.851) \\ Drawer (0.751) } & \shortstack{PandaMobile (0.999) \\ PandaGripper (0.987) \\ HingeCabinet (0.403) \\ SingleCabinet (0.299) \\ FramedWindow (0.289) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.990) \\ Drawer (0.437) \\ Oven (0.395) \\ HingeCabinet (0.377) } & \shortstack{PandaMobile (0.996) \\ HingeCabinet (0.918) \\ PandaGripper (0.881) \\ Toaster (0.612) \\ WallAccessory (0.469) } & \shortstack{PandaMobile (0.997) \\ PandaGripper (0.941) \\ HingeCabinet (0.769) \\ Toaster (0.708) \\ Sink (0.705) } \\
\hline
CloseSingleDoor  & \shortstack{PandaMobile (0.989) \\ SingleCabinet (0.780) \\ Microwave (0.763) \\ PandaGripper (0.697) \\ Wall (0.695) } & \shortstack{Microwave (0.885) \\ PandaMobile (0.872) \\ Oven (0.828) \\ SingleCabinet (0.775) \\ FramedWindow (0.750) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.996) \\ Dishwasher (0.209) \\ Fridge (0.198) \\ CoffeeMachine (0.182) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.998) \\ HingeCabinet (0.431) \\ Box (0.351) \\ Fridge (0.314) } & \shortstack{PandaMobile (0.998) \\ FramedWindow (0.959) \\ PandaGripper (0.879) \\ SingleCabinet (0.805) \\ Oven (0.648) } & \shortstack{Stovetop (1.000) \\ PandaMobile (0.984) \\ FramedWindow (0.907) \\ PandaGripper (0.888) \\ SingleCabinet (0.747) } \\
\hline
CloseDoubleDoor  & \shortstack{PandaMobile (0.994) \\ Wall (0.950) \\ HingeCabinet (0.950) \\ Counter (0.798) \\ PandaGripper (0.571) } & \shortstack{HingeCabinet (0.964) \\ PandaMobile (0.894) \\ PandaGripper (0.798) \\ SingleCabinet (0.657) \\ FramedWindow (0.637) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.988) \\ Hood (0.381) \\ HingeCabinet (0.324) \\ Microwave (0.291) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.994) \\ Oven (0.718) \\ Microwave (0.388) \\ Fridge (0.355) } & \shortstack{PandaMobile (0.996) \\ HingeCabinet (0.913) \\ PandaGripper (0.835) \\ FramedWindow (0.747) \\ Toaster (0.571) } & \shortstack{PandaMobile (0.998) \\ PandaGripper (0.852) \\ Toaster (0.751) \\ HingeCabinet (0.744) \\ Sink (0.736) } \\
\hline
Drawer  &  &  &  &  &  &  \\
\hline
OpenDrawer  & \shortstack{Oven (1.000) \\ Microwave (1.000) \\ FramedWindow (1.000) \\ PandaMobile (0.970) \\ Wall (0.879) } & \shortstack{PandaMobile (0.939) \\ distr\_counter\_2 (0.900) \\ distr\_counter\_1 (0.873) \\ Toaster (0.782) \\ Stovetop (0.753) } & \shortstack{PandaGripper (1.000) \\ Counter (1.000) \\ PandaMobile (0.998) \\ Drawer (0.676) \\ Stool (0.574) } & \shortstack{PandaMobile (1.000) \\ Counter (1.000) \\ PandaGripper (0.999) \\ Drawer (0.775) \\ Dishwasher (0.722) } & \shortstack{Oven (1.000) \\ PandaMobile (0.991) \\ FramedWindow (0.977) \\ Sink (0.938) \\ Toaster (0.681) } & \shortstack{PandaMobile (0.989) \\ Sink (0.885) \\ FramedWindow (0.584) \\ OmronMobileBase (0.491) \\ PandaGripper (0.484) } \\
\hline
CloseDrawer  & \shortstack{Oven (1.000) \\ Microwave (1.000) \\ FramedWindow (1.000) \\ PandaMobile (0.997) \\ Wall (0.852) } & \shortstack{distr\_counter\_2 (0.887) \\ PandaMobile (0.842) \\ PandaGripper (0.781) \\ Toaster (0.718) \\ distr\_counter\_1 (0.712) } & \shortstack{PandaMobile (0.999) \\ Counter (0.999) \\ Drawer (0.996) \\ PandaGripper (0.994) \\ Fridge (0.014) } & \shortstack{PandaMobile (1.000) \\ Counter (1.000) \\ PandaGripper (0.999) \\ Drawer (0.987) \\ Floor (0.013) } & \shortstack{PandaMobile (0.986) \\ FramedWindow (0.811) \\ Sink (0.797) \\ Toaster (0.737) \\ Oven (0.700) } & \shortstack{PandaMobile (0.974) \\ Sink (0.789) \\ PandaGripper (0.590) \\ FramedWindow (0.500) \\ OmronMobileBase (0.467) } \\
\hline
Knobs  &  &  &  &  &  &  \\
\hline
TurnOnStove  & \shortstack{Microwave (1.000) \\ Stove (1.000) \\ PandaMobile (1.000) \\ Stovetop (0.965) \\ Wall (0.941) } & \shortstack{Sink (1.000) \\ Stove (0.999) \\ PandaGripper (0.905) \\ PandaMobile (0.893) \\ Dishwasher (0.813) } & \shortstack{Stove (1.000) \\ PandaMobile (1.000) \\ PandaGripper (0.998) \\ Hood (0.168) \\ Floor (0.123) } & \shortstack{Stove (1.000) \\ PandaMobile (1.000) \\ PandaGripper (1.000) \\ OmronMobileBase (0.216) \\ SingleCabinet (0.167) } & \shortstack{Fridge (1.000) \\ PandaMobile (0.999) \\ PandaGripper (0.912) \\ Microwave (0.641) \\ Stove (0.600) } & \shortstack{PandaMobile (0.994) \\ PandaGripper (0.846) \\ Toaster (0.701) \\ WallAccessory (0.598) \\ Stove (0.543) } \\
\hline
TurnOffStove  & \shortstack{Microwave (1.000) \\ PandaMobile (1.000) \\ Wall (0.999) \\ Stove (0.999) \\ Stovetop (0.952) } & \shortstack{Stove (0.955) \\ Dishwasher (0.931) \\ PandaGripper (0.927) \\ PandaMobile (0.879) \\ Fridge (0.785) } & \shortstack{Stove (1.000) \\ PandaMobile (1.000) \\ PandaGripper (0.993) \\ Floor (0.159) \\ Accessory (0.139) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (1.000) \\ Stove (1.000) \\ Stovetop (0.086) \\ WallAccessory (0.066) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.943) \\ WallAccessory (0.583) \\ Microwave (0.529) \\ Stove (0.493) } & \shortstack{PandaMobile (0.982) \\ PandaGripper (0.913) \\ Sink (0.865) \\ Drawer (0.833) \\ CoffeeMachine (0.587) } \\
\hline
 \end{tabular}
}
\end{table*}



\begin{table*}[t]
\caption{Five most relevant nodes per task and model (Continued).} 
\label{tab:FiveMostRelevantNodesPerTaskAndModel_2}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l}
\shortstack{Task} & 
\multicolumn{2}{|c|}{TopK NR + soft histogram loss} & 
\multicolumn{2}{|c|}{Instruction grounded + NR + soft histogram loss} &
\multicolumn{2}{|c|}{threshold NR + soft histogram loss} \\
\hline
Seed & (1) & (2) & (1) & (2) & (1) & (2)\\
\hline
Lever  &  &  &  &  &  &  \\
\hline
TurnOnSinkFaucet  & \shortstack{PandaMobile (0.999) \\ FramedWindow (0.956) \\ Sink (0.954) \\ Wall (0.864) \\ Counter (0.673) } & \shortstack{PandaMobile (0.930) \\ Fridge (0.851) \\ Sink (0.822) \\ distr\_counter\_1 (0.628) \\ WallAccessory (0.586) } & \shortstack{Sink (1.000) \\ PandaMobile (1.000) \\ PandaGripper (0.995) \\ Stool (0.010) \\ Counter (0.002) } & \shortstack{Sink (1.000) \\ PandaMobile (0.998) \\ PandaGripper (0.995) \\ Stool (0.022) \\ Wall (0.002) } & \shortstack{PandaMobile (1.000) \\ FramedWindow (0.839) \\ Toaster (0.780) \\ PandaGripper (0.735) \\ WallAccessory (0.546) } & \shortstack{PandaMobile (0.996) \\ PandaGripper (0.607) \\ FramedWindow (0.389) \\ distr\_counter\_1 (0.331) \\ distr\_counter\_0 (0.321) } \\
\hline
TurnOffSinkFaucet  & \shortstack{PandaMobile (1.000) \\ Sink (0.956) \\ FramedWindow (0.845) \\ Counter (0.809) \\ Stool (0.797) } & \shortstack{PandaMobile (0.989) \\ distr\_counter\_0 (0.737) \\ distr\_counter\_1 (0.731) \\ PandaGripper (0.686) \\ Sink (0.658) } & \shortstack{PandaMobile (1.000) \\ Sink (1.000) \\ PandaGripper (0.999) \\ HingeCabinet (0.002) \\ Wall (0.000) } & \shortstack{PandaMobile (1.000) \\ Sink (0.999) \\ PandaGripper (0.998) \\ Stool (0.005) \\ Floor (0.002) } & \shortstack{PandaMobile (1.000) \\ FramedWindow (0.971) \\ Fridge (0.919) \\ PandaGripper (0.610) \\ WallAccessory (0.508) } & \shortstack{Toaster (1.000) \\ PandaMobile (1.000) \\ PandaGripper (0.704) \\ FramedWindow (0.560) \\ Fridge (0.527) } \\
\hline
TurnSinkSpout  & \shortstack{PandaMobile (1.000) \\ Sink (0.960) \\ Wall (0.924) \\ FramedWindow (0.879) \\ Counter (0.877) } & \shortstack{PandaMobile (0.980) \\ distr\_counter\_0 (0.838) \\ PandaGripper (0.809) \\ distr\_sink (0.666) \\ distr\_counter\_2 (0.635) } & \shortstack{Sink (1.000) \\ PandaMobile (1.000) \\ PandaGripper (0.998) \\ Counter (0.001) \\ Wall (0.001) } & \shortstack{PandaMobile (1.000) \\ Sink (0.995) \\ PandaGripper (0.954) \\ Floor (0.056) \\ Counter (0.000) } & \shortstack{PandaMobile (1.000) \\ FramedWindow (0.911) \\ PandaGripper (0.887) \\ Sink (0.559) \\ distr\_counter\_0 (0.527) } & \shortstack{PandaMobile (1.000) \\ Fridge (1.000) \\ PandaGripper (0.881) \\ FramedWindow (0.841) \\ WallAccessory (0.651) } \\
\hline
Button  &  &  &  &  &  &  \\
\hline
CoffeePressButton  & \shortstack{PandaMobile (0.999) \\ Counter (0.974) \\ Wall (0.897) \\ PandaGripper (0.857) \\ Fridge (0.741) } & \shortstack{PandaMobile (0.977) \\ PandaGripper (0.941) \\ obj (0.901) \\ CoffeeMachine (0.810) \\ Toaster (0.724) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (1.000) \\ CoffeeMachine (1.000) \\ obj (0.000) \\ WallAccessory (0.000) } & \shortstack{PandaMobile (0.999) \\ PandaGripper (0.989) \\ CoffeeMachine (0.983) \\ obj (0.016) \\ Wall (0.007) } & \shortstack{PandaMobile (0.986) \\ PandaGripper (0.930) \\ Sink (0.820) \\ obj (0.522) \\ WallAccessory (0.495) } & \shortstack{PandaMobile (0.998) \\ FramedWindow (0.961) \\ PandaGripper (0.838) \\ CoffeeMachine (0.667) \\ Toaster (0.644) } \\
\hline
TurnOnMicrowave  & \shortstack{PandaMobile (0.995) \\ Microwave (0.992) \\ Oven (0.983) \\ PandaGripper (0.678) \\ Wall (0.607) } & \shortstack{Toaster (1.000) \\ PandaGripper (0.978) \\ PandaMobile (0.754) \\ Oven (0.728) \\ OmronMobileBase (0.717) } & \shortstack{PandaGripper (0.997) \\ PandaMobile (0.994) \\ Microwave (0.994) \\ Oven (0.014) \\ Counter (0.008) } & \shortstack{Microwave (1.000) \\ PandaMobile (0.999) \\ PandaGripper (0.997) \\ HingeCabinet (0.029) \\ Counter (0.001) } & \shortstack{PandaMobile (0.977) \\ Toaster (0.940) \\ PandaGripper (0.776) \\ Oven (0.425) \\ Microwave (0.249) } & \shortstack{PandaMobile (0.992) \\ PandaGripper (0.619) \\ Microwave (0.222) \\ OmronMobileBase (0.201) \\ CoffeeMachine (0.163) } \\
\hline
TurnOffMicrowave  & \shortstack{Microwave (1.000) \\ PandaMobile (0.999) \\ Oven (0.991) \\ PandaGripper (0.794) \\ Wall (0.622) } & \shortstack{Toaster (0.960) \\ Microwave (0.872) \\ PandaGripper (0.841) \\ Oven (0.815) \\ PandaMobile (0.713) } & \shortstack{PandaGripper (1.000) \\ Microwave (1.000) \\ PandaMobile (1.000) \\ Counter (0.000) \\ WallAccessory (0.000) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.997) \\ Microwave (0.996) \\ HingeCabinet (0.064) \\ WallAccessory (0.000) } & \shortstack{PandaMobile (0.999) \\ PandaGripper (0.873) \\ Toaster (0.768) \\ Oven (0.493) \\ Microwave (0.380) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.867) \\ Microwave (0.256) \\ OmronMobileBase (0.176) \\ Floor (0.132) } \\
\hline
Insertion  &  &  &  &  &  &  \\
\hline
CoffeeServeMug  & \shortstack{PandaMobile (0.997) \\ Wall (0.981) \\ Counter (0.963) \\ Sink (0.760) \\ PandaGripper (0.744) } & \shortstack{CoffeeMachine (0.967) \\ PandaMobile (0.951) \\ obj (0.895) \\ PandaGripper (0.848) \\ Toaster (0.760) } & \shortstack{obj (1.000) \\ CoffeeMachine (1.000) \\ Counter (0.999) \\ PandaMobile (0.995) \\ PandaGripper (0.975) } & \shortstack{CoffeeMachine (1.000) \\ Counter (1.000) \\ PandaMobile (1.000) \\ obj (0.999) \\ PandaGripper (0.986) } & \shortstack{PandaMobile (0.988) \\ Sink (0.924) \\ PandaGripper (0.921) \\ CoffeeMachine (0.846) \\ WallAccessory (0.695) } & \shortstack{PandaMobile (1.000) \\ FramedWindow (0.998) \\ CoffeeMachine (0.958) \\ PandaGripper (0.935) \\ Sink (0.872) } \\
\hline
CoffeeSetupMug  & \shortstack{FramedWindow (0.994) \\ PandaMobile (0.992) \\ Wall (0.981) \\ Counter (0.969) \\ PandaGripper (0.883) } & \shortstack{PandaMobile (0.991) \\ obj (0.989) \\ CoffeeMachine (0.964) \\ PandaGripper (0.917) \\ Toaster (0.722) } & \shortstack{Counter (1.000) \\ CoffeeMachine (0.999) \\ PandaGripper (0.980) \\ PandaMobile (0.974) \\ obj (0.964) } & \shortstack{PandaMobile (1.000) \\ Counter (1.000) \\ CoffeeMachine (1.000) \\ obj (0.995) \\ PandaGripper (0.978) } & \shortstack{FramedWindow (1.000) \\ PandaMobile (0.993) \\ PandaGripper (0.978) \\ CoffeeMachine (0.797) \\ WallAccessory (0.692) } & \shortstack{PandaMobile (1.000) \\ PandaGripper (0.991) \\ CoffeeMachine (0.991) \\ Toaster (0.973) \\ Sink (0.655) } \\
\hline
 \end{tabular}
}
\end{table*}

% \begin{table*}[t]
% \caption{The results represent success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:homogeneous_tasks}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} & 
% \shortstack{Pick and \\ Place (8)} & 
% \shortstack{Open/Close \\ Doors (4)} & 
% \shortstack{Open/Close \\ Drawers (2)} & 
% \shortstack{Twisting \\ Knobs (2)} & 
% \shortstack{Turning \\ Levers (3)} & 
% \shortstack{Pressing \\ Buttons (3)} & 
% \shortstack{Insertion (2)} & 
% \shortstack{Average \\ All Tasks (24)} \\
% \hline
%     & O: Image conf 0.1 &  0.06 & 11.75 &34.0 &9.0 & 39.67 & 12.33 & 3.25 & 12.33  \\
%     & O: Image conf 0.4 &  0.06 & 13.25 &29.0 &8.25 & 35.5 & 12.5 & 1.75 & 11.48  \\
%     & O: BB + Image conf 0.1 &  0.06 & 16.63 &31.5 &11.0 & 34.5 & 9.33 & 3.0 & 12.06  \\
%     & O: BB + Image conf 0.4 &  0.06 & 18.13 &28.75 &12.0 & 35.83 & 10.5 & 3.25 & 12.5  \\
% \hline
% \hline
% \multirow{6}{*}{\rotatebox{90}{\acs{bc}}} & 
%     B: Image & 0.94 & 25.63 & 36.5 & 5.75 & 22.33 & 24.0 & 7.0 & 14.48  \\
%     & B: Point Clouds & 0.0 & 0.0 & 2.0 & 0.25 & 29.33 & 0.0 & 0.13 & 3.96 \\
%     \cline{2-10}
%     & O: Image & 0.13 & 12.63 & 31.5 & 11.75 & 34.5 & 6.0 & 5.75 & 11.25 \\
%     & O: BB + Label & 0.0 & 11.88 & 23.0 & 16.25 & 15.0 & 0.0 & 0.25 & 7.33 \\
%     & O: BB + Image & 0.06 & 9.0 & 24.75 & 6.5 & 36.33 & 5.33 & 3.0 & 9.58 \\
%     & O: Point Clouds &  &  &  &  &  &  &  &  \\
% \hline
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[t]
% \caption{The results represent success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:pnp_tasks}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} & 
% \shortstack{PnPCab \\ ToCounter} & 
% \shortstack{PnPCounter \\ ToCab} & 
% \shortstack{PnPMicrowave \\ ToCounter} & 
% \shortstack{PnPCounter \\ ToMicrowave} & 
% \shortstack{PnPSink \\ ToCounter} & 
% \shortstack{PnPCounter \\ ToSink} & 
% \shortstack{PnPStove \\ ToCounter} & 
% \shortstack{PnPCounter \\ ToStove} & 
% Average \\
% \hline
%     & O: Image conf 0.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.5 & 0.0 & 0.06 \\
%     & O: Image conf 0.4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.5 & 0.0 & 0.0 & 0.06 \\
%     & O: BB + Image conf 0.1 & 0.0 & 0.0 & 0.0 &0.0 & 0.0 & 0.0& 0.0 & 0.5 & 0.06 \\
%     & O: BB + Image conf 0.4 & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.06 \\
% \hline
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[t]
% \caption{The results represent success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:pnp_tasks}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} & 
% \shortstack{PnPCab \\ ToCounter} & 
% \shortstack{PnPCounter \\ ToCab} & 
% \shortstack{PnPMicrowave \\ ToCounter} & 
% \shortstack{PnPCounter \\ ToMicrowave} & 
% \shortstack{PnPSink \\ ToCounter} & 
% \shortstack{PnPCounter \\ ToSink} & 
% \shortstack{PnPStove \\ ToCounter} & 
% \shortstack{PnPCounter \\ ToStove} & 
% Average \\
% \hline
% \multirow{6}{*}{\rotatebox{90}{\acs{bc}}} & 
%     B: Image & 7.0 & 0.0 & 0.0 & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 & 0.94 \\
%     & B: Point Clouds &  0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0  \\
%     \cline{2-11}
%     & O: Image & 0.5 & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.13 \\
%     & O: BB + Label & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
%     & O: BB + Image & 0.5 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.06 \\
%     & O: Point Clouds &  &  &  &  &  &  &  &  &  \\
% \hline
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[t]
% \caption{Drawer tasks: success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:drawer_tasks}
% \centering
% \begin{tabular}{l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} & 
% \shortstack{Close \\ Drawer} & 
% \shortstack{Open \\ Drawer} & 
% Average \\
% \hline
%     & O: Image conf 0.1 & 64.5 & 3.5 & 34.0 \\
%     & O: Image conf 0.4 & 55.5 & 2.5 & 29.0 \\
%     & O: BB + Image conf 0.1 & 59.0 & 4.0  & 31.5 \\
%     & O: BB + Image conf 0.4 & 53.5 & 4.0 & 28.75 \\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \caption{Drawer tasks: success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:drawer_tasks}
% \centering
% \begin{tabular}{l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} & 
% \shortstack{Close \\ Drawer} & 
% \shortstack{Open \\ Drawer} & 
% Average \\
% \multirow{6}{*}{\rotatebox{90}{\acs{bc}}} & 
%     B: Image & 67.5 & 5.5 & 36.5 \\
%     & B: Point Clouds & 4.0 & 0.0 & 2.0 \\
%     \cline{2-5}
%     & O: Image & 57.5 & 5.5 & 31.5 \\
%     & O: BB + Label & 46.0 & 0.0 & 23.0 \\
%     & O: BB + Image & 47.0 & 2.5 & 24.75 \\
%     & O: Point Clouds &  &  &  \\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \caption{Doors tasks: success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:doors_tasks}
% \centering
% \begin{tabular}{l|l|l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} & 
% \shortstack{Close \\ SingleDoor} & 
% \shortstack{Open \\ SingleDoor} & 
% \shortstack{Close \\ DoubleDoor} & 
% \shortstack{Open \\ DoubleDoor} & 
% Average \\
% \hline
%     & O: Image conf 0.1 & 36.0 & 4.0 & 7.0 & 0.0 & 11.75 \\
%     & O: Image conf 0.4 & 40.5 & 4.0 & 8.0 &0.5  & 13.25 \\
%     & O: BB + Image conf 0.1 & 49.0 & 6.5 & 11.0 & 0.0 &16.63  \\
%     & O: BB + Image conf 0.4 & 48.0  & 7.0 & 17.5 & 0.0 & 18.13 \\
% \hline
% \hline
% \multirow{6}{*}{\rotatebox{90}{\acs{bc}}} & 
%     B: Image & 54.5 & 15.5 & 27.0 & 5.5 & 25.63 \\
%     & B: Point Clouds &  0.0 & 0.0 & 0.0 & 0.0 & 0.0  \\
%     \cline{2-7}
%     & O: Image & 38.5 & 9.0 & 3.0 & 0.0 & 12.63 \\
%     & O: BB + Label & 35.5 & 0.0 & 12.0 & 0.0 & 11.88 \\
%     & O: BB + Image & 25.0 & 5.5 & 5.5 & 0.0 & 9.0 \\
%     & O: Point Clouds &  &  &  &  &  \\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \caption{Microwave tasks: success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:microwave_tasks}
% \centering
% \begin{tabular}{l|l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} & 
% \shortstack{TurnOff \\ Microwave} & 
% \shortstack{TurnOn \\ Microwave} & 
% \shortstack{Coffee \\ PressButton} &
% Average \\
% \hline
%     & O: Image conf 0.1 & 19.0 & 15.0 & 3.0 & 12.33 \\
%     & O: Image conf 0.4 & 19.0 & 14.0 & 4.5 & 12.5 \\
%     & O: BB + Image conf 0.1 & 15.5 & 8.5 & 4.0 & 9.33 \\
%     & O: BB + Image conf 0.4 & 19.0 & 8.0 & 4.5 & 10.5 \\
% \hline
% \hline
% \multirow{6}{*}{\rotatebox{90}{\acs{bc}}} & 
%     B: Image & 27.0 & 26.0 & 19.0 & 24.0 \\
%     & B: Point Clouds & 0.0 & 0.0 & 0.0 & 0.0 \\
%     \cline{2-6}
%     & O: Image & 8.0 & 3.0 & 7.0 & 6.0 \\
%     & O: BB + Label & 0.0 & 0.0 & 0.0 & 0.0 \\
%     & O: BB + Image & 2.5 & 5.0 & 8.5 & 5.33 \\
%     & O: Point Clouds &  &  &  &  \\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \caption{Sink tasks: success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:sink_tasks}
% \centering
% \begin{tabular}{l|l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} & 
% \shortstack{TurnOn \\ SinkFaucet} & 
% \shortstack{TurnOff \\ SinkFaucet} & 
% \shortstack{Turn \\ SinkSpout} & 
% Average \\
% \hline
%     & O: Image conf 0.1 & 23.0 & 56.0 & 40.0 & 39.67 \\
%     & O: Image conf 0.4 & 18.5 & 49.5 &38.5  & 35.5 \\
%     & O: BB + Image conf 0.1 & 11.5 & 52.5 & 39.5 & 34.5 \\
%     & O: BB + Image conf 0.4 & 14.0 & 48.5 & 45.0 & 35.83 \\
% \hline
% \hline
% \multirow{6}{*}{\rotatebox{90}{\acs{bc}}} & 
%     B: Image & 15.5 & 22.0 & 29.5 & 22.33 \\
%     & B: Point Clouds & 53.0 & 0.0 & 35.0 & 29.33 \\
%     \cline{2-6}
%     & O: Image & 16.5 & 50.0 & 37.0 & 34.5 \\
%     & O: BB + Label & 10.0 & 9.5 & 25.5 & 15.0 \\
%     & O: BB + Image & 22.0 & 48.5 & 38.5 & 36.33 \\
%     & O: Point Clouds &  &  &  &  \\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \caption{Stove tasks: success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:stove_tasks}
% \centering
% \begin{tabular}{l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} & 
% \shortstack{TurnOn \\ Stove} & 
% \shortstack{TurnOff \\ Stove} & 
% Average \\
% \hline
%     & O: Image conf 0.1 & 11.0 & 7.0 & 9.0 \\
%     & O: Image conf 0.4 & 14.5 & 2.0 & 8.25 \\
%     & O: BB + Image conf 0.1 & 16.0 & 6.0 & 11.0 \\
%     & O: BB + Image conf 0.4 & 15.5 & 8.5 & 12.0 \\
% \hline
% \hline
% \multirow{6}{*}{\rotatebox{90}{\acs{bc}}} & 
%     B: Image & 10.5 & 1.0 & 5.75 \\
%     & B: Point Clouds & 0.0 & 0.5 & 0.25 \\
%     \cline{2-5}
%     & O: Image & 14.5 & 9.0 & 11.75 \\
%     & O: BB + Label & 26.5 & 6.0 & 16.25 \\
%     & O: BB + Image & 6.5 & 6.5 & 6.5 \\
%     & O: Point Clouds &  &  &  \\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \caption{Coffee tasks: success rate over 100 rollouts with 2 models trained on different seeds.}
% \label{tab:coffee_tasks}
% \centering
% \begin{tabular}{l|l|l|l|l}
% \hline
% & \shortstack{Feature \\ Input} &  
% \shortstack{Coffee \\ ServeMug} & 
% \shortstack{Coffee \\ SetupMug} & 
% Average \\
% \hline
%     & O: Image conf 0.1 & 6.5 & 0.0 & 3.25 \\
%     & O: Image conf 0.4 & 3.5 & 0.0 & 1.75 \\
%     & O: BB + Image conf 0.1 & 6.0 & 0.0 & 3.0 \\
%     & O: BB + Image conf 0.4 & 6.5 & 0.0 & 3.25 \\
% \hline
% \hline
% \multirow{4}{*}{\rotatebox{90}{\acs{bc}}} & 
%     B: Image & 11.0 & 3.0 & 7.0 \\
%     & B: Point Clouds & 0.25 & 0.0 & 0.13 \\
%     \cline{2-5}
%     & O: Image & 10.5 & 0.0 & 5.75 \\
%     & O: BB + Label & 0.5 & 0.0 & 0.25 \\
%     & O: BB + Image & 6.0 & 0.0 & 3.0 \\
%     & O: Point Clouds &  &  &  \\
% \hline
% \end{tabular}
% \end{table*}
